Symmetry enhancement in 4d Spin(n) gauge theories and compactification from 6d

We consider a known sequence of dualities involving $4d$ ${\cal N}=1$ theories with $Spin(n)$ gauge groups and use it to construct a new sequence of models exhibiting IR symmetry enhancement. Then, motivated by the observed pattern of IR symmetries we conjecture six-dimensional theories the compactification of which on a Riemann surface yields the $4d$ sequence of models along with their symmetry enhancements, and put them to several consistency checks.

==> sections/sixdim.tex <==
\section{Compactification from six dimensions}
\label{sixdim}

In this section we shall conjecture an explanation for the observed symmetry enhancement. The explanation will be in terms of the compactification of $6d$ SCFTs on a torus with fluxes. In order to understand the logic of the approach we first review the methods introduced in \cite{Kim:2017toz,Kim:2018bpg,Kim:2018lfo} to conjecture $4d$ field theories generated by such compactifications. We start with a $6d$ $\mathcal{N}=(1,0)$ SCFT that we wish to compactify on a torus to four dimensions with fluxes in its global symmetry supported on the torus. The approach generally used to tackle this problem is to compactify first on one circle to $5d$, study the resulting theory and then continue with the compactification to $4d$. The advantage of compactifying first to $5d$ is that it allows us to exploit a relation between $6d$ SCFTs and $5d$ gauge theories.

The specific relation that we seek to exploit is that when compactified on a circle to $5d$, potentially with an holonomy in the global symmetry, the $6d$ SCFT can flow at low-energies to a $5d$ gauge theory. The most well known examples of this are the $\mathcal{N}=(2,0)$ $6d$ SCFTs that reduce to $5d$ maximally supersymmetric Yang-Mills theories \cite{Douglas:2010iu,Lambert:2010iw}. These types of relations are ubiquitous also for $(1,0)$ SCFTs. For instance, the rank $N$ E-string $6d$ SCFTs, compactified on a circle, are known to reduce to the $5d$ $USp(2N)$ gauge theories with an antisymmetric hypermultiplet and eight fundamental hypermultiplets, assuming a suitable holonomy is turned on \cite{Ganor:1996pc}. Similar relations have also been observed for many other $6d$ SCFTs and $5d$ gauge theories, see for instance \cite{Hayashi:2015fsa,Zafrir:2015rga,Hayashi:2015zka,Hayashi:2015vhy}.

Now let us return to the problem at hand, the compactification of a $6d$ $\mathcal{N}=(1,0)$ SCFT on a torus with fluxes in its global symmetry supported on the torus. We would like to first compactify on one circle to $5d$ so that the $6d$ SCFT reduces to a $5d$ gauge theory. However, we need to consider the effect of the flux. This was analyzed in \cite{Kim:2017toz,Kim:2018bpg,Kim:2018lfo}, and the conclusion reached there is that the flux leads to domain walls between different $5d$ gauge theories. The resulting picture is that when we reduce on the first circle to $5d$ we end up with multiple copies of the $5d$ gauge theory description of the $6d$ SCFT interacting through the fields living on the domain walls. Unlike the bulk, the domain walls preserve only half of the supersymmetry, corresponding to $\mathcal{N}=1$ in four dimensions. This corresponds to the fact that the flux preserves only $\mathcal{N}=1$ supersymmetry in $4d$ \cite{Razamat:2016dpl}. Generically the bulk matter is subjected to various $\mathcal{N}=1$ (only) preserving boundary conditions on the domain walls, and these usually reduce the $4d$ $\mathcal{N}=2$ vector and hypermultiplets that are expected to come from the bulk $\mathcal{N}=1$ $5d$ fields to $4d$ $\mathcal{N}=1$ vector and chiral fields, respectively.

We can now reduce along the second circle to $4d$. The $5d$ bulk is straightforward to reduce, as it consists only of IR free gauge theories, and reduces to the same gauge theories in $4d$, though some of the $5d$ bulk matter is killed by Dirichlet boundary conditions on the domain walls. These then interact with one another via the matter living on the domain walls. This chain of thought suggests that the $4d$ theories we get from the compactification of a $6d$ SCFT on a torus with fluxes will resemble a circle of multiple copies of a $4d$ $\mathcal{N}=1$ version of the $5d$ gauge theory. By $\mathcal{N}=1$ version we mean the same gauge theory, but with the $4d$ $\mathcal{N}=2$ vector and hypermultiplets, that are the usual analogues of $5d$ $\mathcal{N}=1$ matter, being replaced by $4d$ $\mathcal{N}=1$ vector and chiral fields. The number of copies is related to the number of domain walls which in turn is related to the value of the flux. In the minimal flux case, we expect just one copy.

We are now ready to discuss the way we shall seek an explanation for the $4d$ symmetry enhancement. For this, we consider $5d$ gauge theories with matter content similar to that of the $4d$ theories we considered, but with $4d$ $\mathcal{N}=1$ vector and chiral fields replaced with $5d$ $\mathcal{N}=1$ vector fields and hypermultiplets. We also consider $6d$ SCFTs that upon circle compactification reduce to these $5d$ gauge theories. Then on one hand, by the preceding picture, it is reasonable that we may be able to get the $4d$ gauge theories we studied in the previous section by the torus compactification with fluxes of the $6d$ SCFTs. On the other hand, the IR $4d$ theory resulting from the compactification should inherit the global symmetry of the $6d$ SCFT, up to the breaking incurred by the flux. Stated in other words, a $6d$ SCFT on a compact manifold with fluxes can be viewed at low enough energies as a $4d$ SCFT with a global symmetry given by the subgroup of the original $6d$ symmetry that commutes with the fluxes. If this symmetry is greater than that visible in the UV $4d$ gauge theory then an enhancement is expected in the IR to conform with the $6d$ expectations. This is the nature of the explanation for the enhancement that we shall propose.

We next turn to analyze this in greater detail. We shall first consider the $5d$ variants of the $4d$ theories we studied in the previous section. Using known results, we argue that they should indeed be low-energy descriptions of $6d$ SCFTs on a circle, and propose a conjecture for the identity of the $6d$ SCFTs in question. We shall then also argue that the global symmetry of these $6d$ SCFTs is such that our proposed explanation can work. We then close the section with describing various aspects of the reduction itself. 

\          

\subsection{Five dimensional analysis}

Here we consider the family of five dimensional $\mathcal{N}=1$ gauge theories given by a $Spin(n+8)$ gauge group, $n$ hypermultiplets in the vector representation and a total of $64$ components of hypermultiplets that are in the spinor representation. This is the $5d$ $\mathcal{N}=1$ version of the $4d$ gauge theories studied in the previous section, modulo gauge singlets. The first thing we note about this family is that it is expected to be a low-energy description of a $6d$ $\mathcal{N}=(1,0)$ SCFT on a circle. To understand how this comes about, it is useful to first recall some aspects of this type of relations. For this, we shall use the example of the $6d$ $\mathcal{N}=(2,0)$ SCFT and $5d$ maximally supersymmetric Yang-Mills theory. The claim here is that the latter still contains some information about the massive Kaluza-Klein excitations. Notably, the $5d$ gauge theory possesses massive non-perturbative excitations given by its instanton particle, and for the case at hand these are supposed to contribute the additional Kaluza-Klein modes.

One way to see that a $5d$ gauge theory may be the low-energy description of a $6d$ $\mathcal{N}=(1,0)$ SCFT on a circle is to find the existence of such modes, particularly, the ones associated with conserved currents. In the $5d$ theory the Kaluza-Klein modes of the $6d$ conserved currents are given by broken conserved current multiplets. This is as the currents are expected to be conserved when the radius of the compactification is taken to zero and we get the $6d$ SCFT on a flat spacetime. In this type of relations, the radius of compactification is inversely related to the coupling constant of the $5d$ gauge theory so the zero radius limit maps to the infinite coupling limit of the gauge theory. Therefore, from the $5d$ gauge theory viewpoint, the only thing breaking the currents is a mass deformation associated with the coupling constant, which has positive mass dimensions in $5d$. This is similar to the phenomena of enhancement of symmetry in $5d$ gauge theories, originally discovered in \cite{Seiberg:1996bd}. In that case the $5d$ gauge theory is a low-energy description of a $5d$ SCFT deformed by a mass deformation. The mass deformation can break the global symmetry whose broken currents manifest in the low-energy gauge theory as instanton particles. The major difference between the two cases is that while in the latter case the low-energy global symmetry plus the instantonic broken currents form a finite Lie group, the global symmetry group of the $5d$ SCFT, in the former case it instead forms an affine Lie group. This affine Lie group essentially describes all the Kaluza-Klein modes of the $6d$ conserved current multiplet. As a result, the appearance of instantonic broken currents in a $5d$ gauge theory whose spectrum is such that they form an affine Lie group is generally an indication that this $5d$ gauge theory is a low-energy description of a $6d$ SCFT on a circle.

In \cite{Tachikawa:2015mha} a method to study the instantonic broken currents provided by $1$-instanton configurations was devised and in \cite{Zafrir:2015uaa} it was used to study cases that include the family of theories that is of interest to us here. It was found there that the resulting spectrum is not consistent with a finite Lie group, but is consistent with an affine one. This is a first indication that this class of theories lift to $6d$ SCFTs, although the analysis there only takes into account broken currents coming from $1$-instanton configurations and so does not see contribution from higher order instantons which could spoil this expected behavior. Nevertheless, ultimately, the question of when does a $5d$ gauge theory possess a UV completion as a $5d$ or $6d$ SCFT is currently unanswered so we cannot say for sure if these gauge theories lift to $6d$ SCFTs or not. However, \cite{Jefferson:2017ahm} has put forward several criteria in an attempt to answer this question. These criteria are known to be insufficient though they do appear to be necessary. The family of theories we study here all fit the criteria for a $6d$ lifting theory. As a result there are several indications that this family lifts to $6d$ SCFTs though it is not assured\footnote{Recently, there has been some progress in the study of $6d$ SCFT lifts of $5d$ gauge theories using geometric methods \cite{ZHM,Jefferson:2018smsm,BJ1,BJ2,ALM,ALLSW1,ALLSW2,ALLSW3,Bhardwaj:2019cls,BJKTV}. It is our hope that these tools may also be useful for the cases discussed here.}.

In what follows we shall assume that this family indeed lifts to $6d$ SCFTs, and try to determine the $6d$ SCFTs it can lift to. Finding a known family of $6d$ $\mathcal{N}=(1,0)$ SCFTs that has the correct properties to reduce to these $5d$ gauge theories, is in itself a non-trivial test that these $5d$ gauge theories are $6d$ lifting. To do this we need to consider what properties do we expect from the $6d$ SCFTs. There are several consistency conditions that should be obeyed. First, the global symmetry of the $6d$ SCFTs must be consistent with that expected from the $5d$ gauge theories when the instantonic broken currents are included. Here we only have partial information as we only know the ones provided by the $1$-instanton. A second requirement is that the Coulomb branch dimension of the $5d$ gauge theory be correctly reproduced by the $6d$ SCFT. Generally, when reducing a $6d$ SCFT on a circle, the Coulomb branch of the resulting $5d$ theory receives contributions from two sources. One is the $6d$ vector multiplets on a circle and the other is the tensor multiplets that are dual to vector multiplets in $5d$. As a result the $5d$ Coulomb branch dimension expected for the low-energy $6d$ SCFT on a circle is given by the sum of the dimension of the $6d$ tensor branch and the total rank of all the gauge groups of the low-energy gauge theory on a generic point on the tensor branch. 

The final test we can perform is to consider the behavior under deformations, notably Higgs branch flows. The Higgs branch has the interesting property of being invariant under a dimensional reduction, and as a result Higgs branch flows done on the $6d$ SCFTs should lead to analogous flows on the $5d$ gauge theories, and vice versa. This can be used as an additional test by flowing from the $5d$ gauge theories to other theories whose lift is known, and seeing if we get the expected $6d$ SCFTs by an analogous flow on the conjectured $6d$ SCFT lifts. It should be noted that while the Higgs branch is invariant under a dimensional reduction, it does change under deformations such as a mass deformation, Coulomb branch or tensor branch vevs, and so the Higgs branch of the SCFT and that of its associated $5d$ or $6d$ gauge theory description may differ (see for instance \cite{Cremonesi:2015lsa,Ferlito:2017xdq,Hanany:2018uhm,HaZ}). Ultimately, the analysis we perform involves some form of deformation of this type and so we do not actually see the entire Higgs branch, which may limit the use of this method.

Next we shall study the global symmetry expected from the $6d$ SCFT based on the $5d$ gauge theory, and use it to conjecture the $6d$ SCFT lift. We then subject that conjecture to various consistency checks. As previously mentioned the global symmetry at the UV, expected from both the classically visible one and the contribution of $1$-instanton states, was studied in \cite{Zafrir:2015uaa}. We summarize the results found there in table \ref{table:gs}. In the table we have also included two other cases involving the $Spin(12)$ gauge group, where the case symmetric under the exchange of the two types of spinors is the one that we naturally associate with the family. This comes about as there is a sequence of Higgs branch flows connecting the theories. Starting from the $Spin(14)$ case, the $Spin(12)$ case we get is the symmetric one. We shall refer to this line, starting with the $Spin(14)$ case, as the main line. The other cases then lie outside it, each starting a new line that joins the main one at $Spin(11)$. We also note that for Lie groups with complex representations we get the twisted affine groups. This implies that the reduction here should be done with a twist that acts like the complex conjugation outer automorphism on these groups.

From these results it is possible to infer the global symmetry of the expected $6d$ SCFT. Specifically, we expect the $6d$ SCFT to have the finite group associated with the affine Lie group. In cases where the group is not affinized at the $1$-instanton level, we assume that this happens at a higher instanton order and we get the same finite Lie group in $6d$. Taking the $5d$ gauge group to be $Spin(n+8)$, we note that the global symmetry of the main line, expected of the $6d$ SCFTs, can be written concisely as $C_{E_{9-n}}\left(SU\left(3\right)\right)\times SU\left(2n\right)$, with the exception of the $n=2$ case where the $SU(4)$ is enhanced to $Spin(7)$.   

\begin{table}[h!]
\begin{center}
\begin{tabular}{|c|c|}
  \hline 
  Theory  & Symmetry  \\
\hline
   $Spin(9)+1V+4S$ & $E^{(2)}_{6}\times SU(2)$ \\ 
\hline
   $Spin(10)+2V+4S$ & $B^{(1)}_{3}\times A^{(2)}_{5}$ \\ 
\hline
   $Spin(11)+3V+2S$ & $A^{(2)}_{5}\times A^{(2)}_{2}\times A^{(2)}_{2}$ \\  
\hline
   $Spin(12)+4V+1S+1C$ & $A^{(2)}_{7}\times A^{(1)}_{1}\times A^{(1)}_{1}\times U(1)^{(2)}$ \\ 
\hline
   $Spin(12)+4V+\frac{3}{2}S+\frac{1}{2}C$ & $A^{(2)}_{2}\times USp(8)$ \\ 
\hline
   $Spin(12)+4V+2S$ & $E^{(2)}_{6}\times A^{(2)}_{2}\times A^{(2)}_{2}$ \\ 
\hline
   $Spin(13)+5V+1S$ & $A^{(2)}_{9}\times A^{(1)}_{1}\times U(1)^{(2)}$ \\
\hline
   $Spin(14)+6V+1S$ & $A^{(2)}_{11}\times A^{(1)}_{1}$ \\ 
\hline
\end{tabular}
 \end{center}
\label{table:gs}
\caption{The minimal symmetry consistent with the perturbative plus $1$-instanton contribution for the $5d$ $Spin$ gauge theories considered here. The spectrum of the expected additional current is such that it can only be accommodated by an affine group, at least for some factors of the global symmetry. This is interpreted as the theory lifting to a $6d$ SCFT in the infinite coupling limit, whose symmetry is the finite Lie group associated with the affine case. The superscript here denotes whether the affine group is the twisted ($2$) or the untwisted version ($1$). This lifts to whether the compactification of the $6d$ SCFT involves a twist or not. We also use the notation of $U(1)^{(2)}$ for a $U(1)$ group projected out by charge conjugation.}
\end{table}        

This enables us to formulate a conjecture for the identity of the $6d$ SCFTs in question. Specifically, we conjecture that the $6d$ SCFT lifts have tensor branch descriptions given by a gauging of the rank $1$ E-string theory by a pure $SU(3)$ gauge group and an additional $SU(n)$ gauge group with $2n$ hypermultiplets in the fundamental representation. This combination of matter gives an anomaly free theory, once tensor multiplets are introduced for the two gauge groups and used to cancel their respective gauge anomalies. Therefore, we expect it to be a low-energy description of a $6d$ SCFT, deformed by going on the tensor branch associated with the coupling constants of the two gauge groups. This $6d$ SCFT is our conjectured UV completion of the $Spin(n+8)$ family of theories.

This conjecture indeed reproduces the desired global symmetry as we get the $SU\left(2n\right)$ from the symmetry rotating the $2n$ fundamental hypermultiplets, and $C_{E_{9-n}}\left(SU\left(3\right)\right)$ is by definition the commutant of $SU(3)\times SU(n)$ inside $E_8$. Here the $U(1)$ baryon symmetry naively expected from the fundamental hypermultiplets is anomalous and so is not actually a global symmetry. The only exceptional case is the $n=2$ case as now we have an $SU(2)$ gauge theory with four fundamental hypermultiplets. Because the fundamental representation of $SU(2)$ is self-conjugate, the $SU(4)$ symmetry we naively expect to rotate four complex hypermultiplets is enhanced. Naively we expect it to enhance to $SO(8)$, but as discussed in \cite{Ohmori:2015pia}, it turns out that the SCFT only exhibits a $Spin(7)$ symmetry. Therefore, in this case we expect the global symmetry to be $Spin(7)\times SU(6)$, in accordance with the symmetry expected from the associated $5d$ gauge theory. 

Another noteworthy case is the $n=1$ case. Here we naively have an $SU(1)$ gauging of the rank $1$ E-string theory. Here the $SU(1)$ part is really just the tensor multiplet that always accompanies any gauge group in low-energy gauge theories related to $6d$ SCFTs on the tensor branch. This tensor joins with the rank $1$ E-string tensor to give the rank $2$ E-string SCFT. As a result, this case is better described as an $SU(3)$ gauging of the rank $2$ E-string SCFT. This is indeed an anomaly free theory, once a tensor multiplet is introduced for the $SU(3)$ gauge group and used to cancel the $SU(3)$ gauge anomalies, and should descend from a $6d$ SCFT deformed by a vev to the scalar in the tensor multiplet.   

After we saw that our conjecture correctly reproduces the expected global symmetry we next consider other evidence for it. First we note that the end point of the main line is the same for both the $5d$ and $6d$ theories. Notably, we cannot have $64$ spinor degrees of freedom for $Spin(n+8)$ if $n>6$ and likewise it is impossible to embed $SU(3)\times SU(n)$ inside $E_8$ if $n>6$. We also note that the Coulomb branch of the $5d$ theories agrees with that expected from the $6d$ SCFTs. Before explaining this, we should first consider the $5d$ reduction in greater detail. Specifically, we noted that in $5d$ we see twisted affine groups. This suggests that the reduction must be done with a discrete symmetry twist which acts on these groups through their charge conjugation outer automorphism. There is a natural candidate for this discrete symmetry. Specifically, the $6d$ semi-gauge theory has a discrete symmetry acting on all the matter through charge conjugation, and it is natural to conjecture that it is present also in the $6d$ SCFT. In that case the $5d$ reduction should be done with a twist using that symmetry. 

We can now return to comparing the expected Coulomb branch dimension. As previously mentioned, when we compactify a $6d$ SCFT on a circle the Coulomb branch of the resulting $5d$ theory gets contributions from both the tensor branch and the vector multiplets on the circle, where the latter are also affected by the twist. The tensor branch of all the $6d$ SCFTs in the main line is three dimensional, so the Coulomb branch dimension of the expected $5d$ theory should be three plus the rank of the gauge symmetry invariant under the twist. Given a vector multiplet, we can parametrize the Coulomb branch by operators of the form $Tr(\phi^i)$, where $\phi$ is the scalar in the vector multiplet, which in our case comes from the component of the $6d$ vector in the circle direction. It is well known that for groups of type $SU(n)$, there are $n-1$ independent such operators, given by $i=2,3,4,...,n$. Out of these, the cases with $i$ even are invariant under the charge conjugation outer automorphism while cases with $i$ odd are not. When we compactify with a charge conjugation twist, only the cases that are invariant under the twist contribute to the Coulomb branch dimension. As a result, we expect one contribution from the $SU(3)$ vector multiplet, and $\frac{n}{2}$ or $\frac{n-1}{2}$ from the $SU(n)$ vector multiplet, depending on whether $n$ is even or odd.

Summing all the contributions we expect the Coulomb branch of the resulting $5d$ theory to be $4+\frac{n}{2}$ for $n$ even or $4+\frac{n-1}{2}$ for $n$ odd. We can next compare it with the proposed $5d$ gauge theory. For a $Spin(n+8)$ gauge theory, the Coulomb branch dimension should be given by the rank of the gauge group, which is indeed $4+\frac{n}{2}$ for $n$ even or $4+\frac{n-1}{2}$ for $n$ odd.

Another check we can do is to consider Higgs branch flows. As we previously mentioned, the main line is connected via one such flow, where we give a vev to the gauge invariant made from a $Spin(n+8)$ vector hyper. We expect a similar flow pattern also for the $6d$ theories, and indeed such a flow pattern exists. Specifically, we can give a vev to a meson of the  $SU(n)$ group breaking it to $SU(n-1)$. This indeed initiates an analogous flow pattern. Interestingly, we can continue this line past the $n=1$ case. Recall that for $n=1$ we had a $Spin(9)$ $5d$ gauge theory with a single vector hyper and four spinor hypers. We can give a vev to the vector in the $Spin(9)$ theory leading to a $5d$ $Spin(8)$ gauge theory with four spinor hypers of both chiralities. We next consider the analogous flow in the conjectured $6d$ lift, which for this case is an $SU(3)$ gauging of the rank $2$ E-string theory. In this $6d$ SCFT, this Higgs branch flow should match giving a vev to the moment map operator associated with the $SU(2)$ global symmetry, which is the one reducing to the operator we gave a vev to in the $5d$ $Spin(9)$ gauge theory. This vev is known to break the rank $2$ E-string theory to two decoupled copies of the rank $1$ E-string theory. This suggests that the $5d$ $Spin(8)$ gauge theory with four spinor hypers of both chiralities lifts to a twisted compactification of a $6d$ SCFT with a tensor branch description as an $SU(3)$ gauging of two rank $1$ E-string theories, also known as the minimal $(E_6,E_6)$ conformal matter SCFT \cite{ZHTV}. 

This proposal can again be checked using similar methods as the previous case. First, we note that the $5d$ $Spin(8)$ gauge theory with four spinor hypers of both chiralities appears to be $6d$ lifting according to the criteria of \cite{Jefferson:2017ahm}. Also, it was found to have a perturbative plus 1-instanton spectrum of currents that is consistent with $E^{(2)}_6 \times E^{(2)}_6$ \cite{Zafrir:2015uaa}. Finally, we note that the Coulomb branch dimension matches that expected from the $6d$ SCFT. In light of this proposal, we can wonder whether an interesting enhancement of symmetry can be found in a $4d$ $\mathcal{N}=1$ $Spin(8)$ gauge theory with four spinor chirals of both chiralities, one that can then be also attributed to a similar $6d$ origin. We indeed find such a case which is further discussed in the appendix. 

One can also consider other flows, notably ones that in the $5d$ theory are associated with spinor vevs. For instance we can consider giving a spinor vev to one of the spinors in the $5d$ $Spin(8)$ gauge theory with four spinor hypers of both chiralities that we introduced previously. This just leads to a $5d$ $Spin(7)$ gauge theory with four spinor hypers and three vector hypers, as can be seen by using the triality automorphism of $Spin(8)$ to map the spinor vev to a vector one. This $5d$ gauge theory appeared already in \cite{Razamat:2018gbu}, where it was conjectured that it is $6d$ lifting and lifts to a twisted compactification of a $6d$ SCFT with tensor branch description as a gauging of a rank $1$ E-string SCFT by an $SU(3)$ gauge theory with six fundamental hypermultiplets. We can now see that this conjecture is compatible with our results. Specifically, the spinor vev we consider here should map to going on the Higgs branch of one of the rank $1$ E-string theories, where the choice of E-string theory mapping to the choice of the chirality of the spinor given a vev. This should then break the rank $1$ E-string theory to free hypers, which just become six fundamentals for the $SU(3)$ gauge group. We can similarly consider other spinor vevs, however, as this can be long and quite technical, we shall not discuss it in detail here. 

Finally, we want to consider the two other $Spin(12)$ theories. We can also find proposed $6d$ SCFT lifts for these cases. For the case with three half-hyper spinors in one chirality and one in the other, we propose the $6d$ lift is given again by a rank $1$ E-string theory gauged by a pure $SU(3)$ gauge theory, but also by a $G_2$ gauge theory with four fundamental hypermultiplets. For the case with spinor hypers of only one chirality we propose the $6d$ lift is given again by two rank $1$ E-string theories, both gauged by a pure $SU(3)$ gauge theory with an additional pure $SU(3)$ gauge theory gauging only one of them. When the appropriate tensors are added, both give anomaly free gauge theories, which should lift to $6d$ SCFTs. The resulting $6d$ SCFTs should have a global symmetry compatible with the $5d$ gauge theories. It is also straightforward to see that the resulting Coulomb branch dimensions match that expected from the $5d$ gauge theory. Finally both of these posses a Higgs branch flow leading to the main branch. In the former case, it is given by Higgsing the $G_2$ to $SU(3)$, while in the latter it is given by going on the Higgs branch of the rank $1$ E-string SCFT, gauged by only one $SU(3)$. This breaks the rank $1$ E-string SCFT to free hypermultiplets, some of which decouple, but those that do not become six fundamental hypermultiplets for the gauging $SU(3)$ group.    

\

\subsection{Aspects of the reduction}

Having formulated a conjecture for the $6d$ lift of the family of $Spin(n+8)$ gauge theories, we now want to use this conjecture to propose a general explanation for the origin of the $4d$ symmetry enhancement pattern \eqref{4dpatt8} found in the previous section. The idea is as follows. Consider a compactification of these theories on a torus with fluxes in the global symmetry. As we pointed out the global symmetry in this class of theories is $C_{E_{9-n}}\left(SU\left(3\right)\right)\times SU\left(2n\right)$, except for $n=2$. This global symmetry is expected to be inherited by the $4d$ theory, though part of it may be broken by the flux and other discrete options having to do with coupling to non-trivial flavor backgrounds (see for instance \cite{Bah:2017gph,Ohmori:2018ona}). Specifically, let us concentrate on flux, and consider turning on two independent fluxes, one in a $U(1)$ such that $SU\left(2n\right)$ is broken to $U(1)\times SU\left(n\right)^2$ and another in $C_{E_{9-n}}\left(SU\left(3\right)\right)$ such that it is broken to $U(1)\times C_{E_{9-n}}\left(SU\left(3\right)\times SU\left(2\right)\right)$. This should lead to a $4d$ theory with a global symmetry which is at least $U(1)^2\times C_{E_{9-n}}\left(SU\left(3\right)\times SU\left(2\right)\right) \times SU\left(n\right)^2$. We include here the possibility that one or both of these fluxes are zero and the symmetry enhances.

From the resulting $4d$ theories, we can generate additional theories by various deformations, like mass deformations, giving vevs to various operators or coupling to various additional free fields. In particular it is possible to use these deformations to get to a theory with $U(1)\times C_{E_{9-n}}\left(SU\left(3\right)\times SU\left(2\right)\right) \times SU\left(n\right)^2$ global symmetry, where one $U(1)$ is broken by the deformation. It is also possible to cause the breaking of the $6d$ global symmetry to this symmetry using the deformations instead of the fluxes. We note that the global symmetry $U(1)\times C_{E_{9-n}}\left(SU\left(3\right)\times SU\left(2\right)\right) \times SU\left(n\right)^2$ is the enhanced symmetry we found in the $4d$ $Spin(n+8)$ models, see Eq. \eqref{4dpatt8}. The only exceptional case is the $n=2$ one where, on one side the $6d$ global symmetry is enhanced, while on the other the $4d$ found enhanced symmetry is smaller. Presumably this should be accounted for by the deformation incidentally breaking more symmetry in this case. The matter content of these $Spin(n+8)$ models is, up to additional free fields, precisely an $\mathcal{N}=1$ $4d$ version of the matter content of the $5d$ theory we get via a twisted circle compactification. By our previous considerations then, it seems quite reasonable that these theories could arise from deformations of the $6d$ compactifications, and thus the enhancement of symmetry in them can be explained in this way.

We note that to get the $5d$ theories we need to perform a charge conjugation twist. This may explain why there is a rank enhancement. The general logic here is to build this theory by gluing two tubes each incorporating the charge conjugation twist. As each tube incorporates a twist, the punctures at the end should be described by boundary conditions for the twisted theory, that is the $5d$ $Spin(n+8)$ theories. The rank of the global symmetry visible in these theories is smaller than that of the $6d$ SCFT because of the twist. When we glue together two of these tubes we expect, on one hand, to get $4d$ $Spin(n+8)$ models with a matter content similar to the $4d$ theories considered here, though these in general will contain additional fields. On the other hand, as we are joining two tubes with a $\mathbb{Z}_2$ twist, the twist in the full surface vanishes and the symmetry should enhance back to the full $6d$ global symmetry compatible with the flux. This then leads to a large enhancement of symmetry in this theory and its descendants through various deformations preserving this symmetry.

This matching in behavior between the $4d$ enhanced symmetries and the global symmetries of the $6d$ SCFT lifts of the $\mathcal{N}=1$ $5d$ variants is the major indirect evidence for our proposed explanation. Unfortunately, as the symmetry of our $4d$ models is smaller than that of the direct compactification, some deformations must also be involved, though precisely which ones is unknown. Furthermore, from the models discussed here, it is possible to generate new ones with the same enhanced symmetry by flipping operators in complete representations of the enhanced groups. The choice of flipping we used in $4d$ is partially dictated by the desire to avoid having operators hitting the unitarity bound. However, this restriction is usually not obeyed in the torus compactifications of $6d$ SCFTs. The large number of possibilities regarding the uncertainties in the details of the $6d$ compactification makes it difficult to quantitatively check this proposal by, for example, anomaly computations. We do note that there are similar cases of enhancements, like the ones discussed in \cite{Razamat:2018gbu}, where some of the enhancements have been linked also quantitatively to a $6d$ reduction. In these cases the torus compactifications of the $6d$ SCFTs in question are better understood, allowing one to explicitly find the needed deformations. For now, we leave a more detailed study of this proposal for future work.    


